On the ratio of total masses of species to resources for a logistic equation with Dirichlet boundary condition

We consider the stationary problem for a diffusive logistic equation with the homogeneous Dirichlet boundary condition. Concerning the corresponding Neumann problem, Wei-Ming Ni proposed a question as follows: Maximizing the ratio of the total masses of species to resources. For this question, Bai, He and Li showed that the supremum of the ratio is 3 in the one dimensional case, and the author and Kuto showed that the supremum is infinity in the multi-dimensional ball. In this paper, we show the same results still hold true for the Dirichlet problem. Our proof is based on the sub-super solution method and needs more delicate calculation because of the range of the diffusion rate for the existence of the solution.

==> discussion.tex <==
In this section, we give some concluding remarks.
For each dimension number $n \ge 1$ and any $(d,m) \in (0,\infty) \times L_+^{\infty}(B_1^n)$, we define
\[ I_n(d,m) := \dfrac{\| \udm \|_{L^1(B_1^n)}}{\|m\|_{L^1(B_1^n)}}, \]
where $B_1^n = \{\,x \in \R^n \mid |x|<1 \,\}$.
Concerning the maximizing problem
\[ M_n := \sup_{(d,m) \in (0,\infty) \times L_+^{\infty}(B_1^n) } I_n(d,m), \]
Theorem \ref{main_thm} reveals a fact that $M_n = \infty$ if $n \ge 2$, which is a big contrast to the one-dimensional situation $M_1 = 3$ obtained by \cite{BaiHeLi}.

In the one-dimensional case when $n = 1$, a maximizing sequence $(\dep, \mep)=(\sqrt{\e}, \e^{-1} \chi_{[0,\e]})$ realizes $I(\dep, \mep) \nearrow M_1 = 3$ as $\e \to +0$ (\cite{BaiHeLi}), where $\chi_{A}$ denotes the characteristic function of the set $A$.
This result says that, under the concentration setting of resource as $\mep = \e^{-1}\chi_{[0,\e]}$, a small control of the diffusion rate as $\dep = \sqrt{\e}$ can make $I_1(\dep, \mep)$ tend to the supremum $3$ from below as $\e \to +0$.
In this situation as $\e \to +0$, the profile of $\uep(x)$ obtained by \cite{Inoue} shows that $\uep(x)$ with $x \in [0,\e]$ grows with the order $O(1/\sqrt{\e})$.
This result means that the species in the resource interval $[0,\e]$ cannot follow the height (the $L^{\infty}$ norm) $1/\e$ of resource.
Furthermore, the singular limit $\dep = \sqrt{\e} \to 0$ leads to the shrink property that $\uep(x) \to 0$ uniformly in any compact set contained in $(0,1]$ as $\e \to +0$.

In the two-dimensional case when $n = 2$, Theorem \ref{mainthm2} asserts that, under the concentration of resource near the center as $\mep = \e^{-2} \chi_{B_\e^2}$, a middle control of the diffusion rate as $\dep = c_1$ (independent of $\e$) can make $I_2(c_1, \mep)$ tend to infinity as $\e \to +0$.
Furthermore, the profile of the sub-solution $\underline{\uep} = c_2 \e^{-2}\exp(-(|x|/\e)^2)$ for $x \in \overline{B_\e^2}$ ensures that $\uep(x) (\, \ge \underline{u}_{\e}(x)\,)$ for $x \in \overline{B_\e^2}$ grows with the order $O(1/\e^{2})$ as $\e \to +0$.
This fact means that the species in the resource disk $B_\e^2$ can follow the height (the $L^\infty$ norm) $1 / \e^2$ of resource.
On the other hand, in the no-resource annulus
$B_1^2 \setminus B_\e^2$, the sub-solution $\underline{u}_{\e}(x) = c_2 e^{-1}|x|^{-2}$ for $x \in \overline{B_1^2} \setminus \overline{B_\e^2}$ implies that $\uep(x) \ge \underline{u}_{\e}(x)$ for $x \in \overline{B_1^2} \setminus \overline{B_\e^2}$.
This fact is also a big difference from the one-dimensional case that $\uep(x)$ decays to zero in any compact set contained in $(0,1]$ as $\e \to +0$.

In the higher dimensional case when $n \ge 3$, under the concentration of resource as $\mep = \e^{-n} \chi_{B_\e^n}$, a large control of the diffusion rate as $\dep = c_1 / \e^{n-2}$ can make $I_n(\dep, \mep)$ tend to infinity as $\e \to +0$.
In this situation as $\e \to +0$, the profile of the sub-solution $\underline{u}_{\e}(x)$ tells us that $\uep(x)$ can follow $\mep(x)$ in the resource ball $\overline{B_\e^n}$ with the same order $O(1/\e^{n})$ and $\uep(x) \ge \underline{u}_{\e}(x)=c_2 e^{-1} |x|^{-n}$ for the no-resource region $\overline{B_1^n} \setminus \overline{B_\e^n}$.

As another point of view, we consider the following integral equation which $(\uep, \dep, \mep)$ satisfies:
\begin{equation}\label{int-eq1}
  \dep \uep = (-\Delta +I)^{-1} [\uep (\mep(x)+\dep-\uep)],
\end{equation}
where $(-\Delta +I)^{-1}$ denotes the inverse operator of $-\Delta +I \,:\, W^{2,2}(B_1^n) \to L^2(B_1^n)$ with homogeneous Neumann boundary condition on $\partial B_1^n$.
Hence \eqref{int-eq1} is expressed as
\begin{equation}\label{int-eq2}
  \dep \uep(x) = \int_{B_1^n} G(|x-y|) \uep(y) (\mep(y)+\dep-\uep(y)) \,dy,
\end{equation}
where $G(r)$ is a corresponding Green function whose asymptotic growth order as $r \to +0$ is known as follows
\[ G(r) = \begin{cases}
O(r) &(n=1),\\
O(|\log r|) &(n=2),\\
O(1/r^{n-2}) &(n\ge 3).
\end{cases} \]

In the one-dimensional case $n=1$, since $(\dep, \mep) = (\sqrt{\e}, \e^{-1} \chi_{[0,\e]})$, then \eqref{int-eq2} implies
\begin{equation}\label{1d-int}
  \sqrt{\e} \uep(0) = \int_0^\e G(x)\uep(x) \biggl( \frac{1}{\e}+\sqrt{\e}-\uep(x) \biggr) \,dx + \int_\e^1 G(x)\uep(x) (\sqrt{\e}-\uep(x)) \,dx.
\end{equation}
By the boundedness of $G(x)=O(x)$ as $x \to +0$ and the growth order $\uep(x) = O(1/\sqrt{\e})$ for $x \in [0,\e]$ as $\e \to +0$, we see that the integral over $[\e, 1]$ is a main term in the right-hand side of \eqref{1d-int}.

In the two-dimensional case $n=2$, \eqref{int-eq2} implies that $U_{\e}(r) := \uep(x) \;(r=|x|)$ satisfies
\begin{equation}\label{int-eq3}
  \begin{split}
    c_1 U_{\e}(0) =& 2\pi\int_0^\e rG(r)U_{\e}(r) \biggl( \frac{1}{\e^2}+c_1-U_{\e}(r) \biggr) \,dr \\
    & +2\pi\int_\e^1 rG(r)U_{\e}(r)(c_1-U_{\e}(r)) \,dr.
  \end{split}
\end{equation}
Here we recall that
\[ \frac{c_2}{\e^2} e^{-r^2/\e^2} \le U_{\e}(r) \le \frac{1}{\e^2} \quad\text{for}\; r \in [0,\e]. \]
Together with $G(r) = O(|\log r|)$ as $r \to +0$, one can verify that the integral over $[0,\e]$ is a main term in the right-hand side of \eqref{int-eq3}.
%and $1/\e^2-U_{\e}(\e)$ remains bounded as $\e \to +0$.

In the higher dimensional case $n \ge 3$, \eqref{int-eq2} implies
\begin{equation}\label{int-eq4}
  \begin{split}
    \frac{c_1}{\e^{n-2}} U_{\e}(0) =& A_n \int_0^\e r^{n-1}G(r)U_{\e}(r) \biggl( \frac{1}{\e^n}+\frac{c_1}{\e^{n-2}}-U_{\e}(r) \biggr) \,dr\\
    & +A_n \int_\e^1 r^{n-1}G(r)U_{\e}(r) \biggl( \dfrac{c_1}{\e^{n-2}}-U_{\e}(r) \biggr) \,dr.
  \end{split}
\end{equation}
By virtue of facts that
\[ \frac{c_2}{\e^n} e^{-r^n/\e^n} \le U_{\e}(r) \le \frac{1}{\e^n} \quad\mbox{for}\; r \in [0,\e] \]
and $G(r) = O(1/r^{n-2})$ as $r \to +0$, one can see that the integral over $[0,\e]$ is a main term in the right-hand side of \eqref{int-eq4} since the order of the left-hand side is equal to $O(1/\e^{2(n-1)})$.

By these facts for each dimensional case, we can say that the difference of the growth order of $G(r)$ as $r \to +0$ depending on $n$ strongly influences on that of the profile of $\uep$ depending on $n$.
From such a view-point,
more detailed profile of $\uep$ will be discussed elsewhere.

